Your Model is Overconfident, and Other Lies We Tell Ourselves

The difficulty intrinsic to a given example, rooted in its inherent ambiguity, is a key yet often overlooked factor in evaluating neural NLP models. We investigate the interplay and divergence among various metrics for assessing intrinsic difficulty, including annotator dissensus, training dynamics, and model confidence. Through a comprehensive analysis using 29 models on three datasets, we reveal that while correlations exist among these metrics, their relationships are neither linear nor monotonic. By disentangling these dimensions of uncertainty, we aim to refine our understanding of data complexity and its implications for evaluating and improving NLP models.

==> Figures/heatmap.tex <==
\begin{figure*}%[ht]
    \centering
    % First row
    \begin{subfigure}[b]{0.23\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Figures/quant5_model_population_entropy.newlabel.png}%
        \caption{$\mathbb{M}_{\text{ent}}^{\neg\mathrm{ref}}$ vs $\mathbb{H}_{\text{ent}}$}
    \end{subfigure}%\hfill
    \begin{subfigure}[b]{0.23\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Figures/quant5_model_dissensus.newlabel.png}%
        \caption{$\mathbb{M}_{\text{dis}}^{\neg\mathrm{ref}}$ vs $\mathbb{H}_{\text{ent}}$}
    \end{subfigure}%\hfill
    \begin{subfigure}[b]{0.23\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Figures/quant5_avg_model_entropy.newlabel.png}%
        \caption{$\mathbb{M}_{\text{avg\ ent}}^{\neg\mathrm{ref}}$ vs $\mathbb{H}_{\text{ent}}$}
    \end{subfigure}
    \hfill
    
    % Second row
    \begin{subfigure}[b]{0.23\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Figures/quant5_avg_xtrain_avg_failure.newlabel.png}%
        \caption{$\mathbb{M}_{\text{avg\ ckpt}}^{+\mathrm{ref}}$ vs $\mathbb{H}_{\text{ent}}$}
    \end{subfigure}
    \begin{subfigure}[b]{0.23\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Figures/quant5_avg_failure.newlabel.png}%
        \caption{$\mathbb{M}_{\text{fail}}^{+\mathrm{ref}}$ vs $\mathbb{H}_{\text{ent}}$}
    \end{subfigure}
    \begin{subfigure}[b]{0.23\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Figures/quant5_avg_xtrain_nextok_success.newlabel.png}
        \caption{$\mathbb{M}_{1^{\text{st}}\ ckpt}^{+\mathrm{ref}}$ vs $\mathbb{H}_{\text{ent}}$}
    \end{subfigure}
    \begin{subfigure}[b]{0.23\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Figures/quant5_avg_layer_all_next_correct.newlabel.png}
        \caption{$\mathbb{M}_{1^{\text{st}}\ layer}^{+\mathrm{ref}}$ vs $\mathbb{H}_{\text{ent}}$}
    \end{subfigure}

    \caption{Heatmap Analysis}
    \label{fig:heat}
\end{figure*}

==> Figures/histplot.tex <==
\begin{figure*}%[ht]
    \centering
    % First row
    \begin{subfigure}[b]{0.23\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Figures/data_model_population_entropy.newlabel.png}%
        \caption{$\mathbb{M}_{\text{ent}}^{\neg\mathrm{ref}}$ vs $\mathbb{H}_{\text{ent}}$}
    \end{subfigure}%\hfill
    \begin{subfigure}[b]{0.23\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Figures/data_model_dissensus.newlabel.png}%
        \caption{$\mathbb{M}_{\text{dis}}^{\neg\mathrm{ref}}$ vs $\mathbb{H}_{\text{ent}}$}
    \end{subfigure}%\hfill
    \begin{subfigure}[b]{0.23\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Figures/data_avg_model_entropy.newlabel.png}%
        \caption{$\mathbb{M}_{\text{avg\ ent}}^{\neg\mathrm{ref}}$ vs $\mathbb{H}_{\text{ent}}$}
    \end{subfigure}
    \hfill
    
    % Second row
    \begin{subfigure}[b]{0.23\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Figures/data_avg_xtrain_avg_failure.newlabel.png}%
        \caption{$\mathbb{M}_{\text{avg\ ckpt}}^{+\mathrm{ref}}$ vs $\mathbb{H}_{\text{ent}}$}
    \end{subfigure}
    \begin{subfigure}[b]{0.23\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Figures/data_avg_failure.newlabel.png}%
        \caption{$\mathbb{M}_{\text{fail}}^{+\mathrm{ref}}$ vs $\mathbb{H}_{\text{ent}}$}
    \end{subfigure}
    \begin{subfigure}[b]{0.23\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Figures/data_avg_xtrain_nextok_success.newlabel.png}
        \caption{$\mathbb{M}_{1^{\text{st}}\ ckpt}^{+\mathrm{ref}}$ vs $\mathbb{H}_{\text{ent}}$}
    \end{subfigure}
    \begin{subfigure}[b]{0.23\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Figures/data_avg_layer_all_next_correct.newlabel.png}
        \caption{$\mathbb{M}_{1^{\text{st}}\ layer}^{+\mathrm{ref}}$ vs $\mathbb{H}_{\text{ent}}$}
    \end{subfigure}

    \caption{Histplot Analysis}
    \label{fig:hist}
\end{figure*}

==> Figures/residual.tex <==
\begin{figure*}%[ht]
    \centering
    % First row
    \begin{subfigure}[b]{0.23\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Figures/resid_model_population_entropy.newlabel.png}%
        \caption{$\mathbb{M}_{\text{ent}}^{\neg\mathrm{ref}}$ vs $\mathbb{H}_{\text{ent}}$}
    \end{subfigure}%\hfill
    \begin{subfigure}[b]{0.23\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Figures/resid_model_dissensus.newlabel.png}%
        \caption{$\mathbb{M}_{\text{dis}}^{\neg\mathrm{ref}}$ vs $\mathbb{H}_{\text{ent}}$}
    \end{subfigure}%\hfill
    \begin{subfigure}[b]{0.23\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Figures/resid_avg_model_entropy.newlabel.png}%
        \caption{$\mathbb{M}_{\text{avg\ ent}}^{\neg\mathrm{ref}}$ vs $\mathbb{H}_{\text{ent}}$}
    \end{subfigure}
    \hfill
    
    % Second row
    \begin{subfigure}[b]{0.23\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Figures/resid_avg_xtrain_avg_failure.newlabel.png}%
        \caption{$\mathbb{M}_{\text{avg\ ckpt}}^{+\mathrm{ref}}$ vs $\mathbb{H}_{\text{ent}}$}
    \end{subfigure}
    \begin{subfigure}[b]{0.23\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Figures/resid_avg_failure.newlabel.png}%
        \caption{$\mathbb{M}_{\text{fail}}^{+\mathrm{ref}}$ vs $\mathbb{H}_{\text{ent}}$}
    \end{subfigure}
    \begin{subfigure}[b]{0.23\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Figures/resid_avg_xtrain_nextok_success.newlabel.png}
        \caption{$\mathbb{M}_{1^{\text{st}}\ ckpt}^{+\mathrm{ref}}$ vs $\mathbb{H}_{\text{ent}}$}
    \end{subfigure}
    \begin{subfigure}[b]{0.23\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Figures/resid_avg_layer_all_next_correct.newlabel.png}
        \caption{$\mathbb{M}_{1^{\text{st}}\ layer}^{+\mathrm{ref}}$ vs $\mathbb{H}_{\text{ent}}$}
    \end{subfigure}

    \caption{Residual Analysis}
    \label{fig:resi}
\end{figure*}

==> Tables/dynasent-results/spearman-vs-h-ent-1b.tex <==
\begin{tabular}{l  S[table-format=2.4] S[table-format=2.4] S[table-format=2.4] S[table-format=2.4] } %r rrr r rrrr} % <================================ p{6cm}
\toprule
 & \multicolumn{2}{c}{re-balanced} & \multicolumn{2}{c}{original} \\
 & {{soft}} & {{hard}} & {{soft}} & {{hard}} \\
\midrule
$\mathbb{M}_\mathrm{dis}$ &  0.155306  & 0.143457  &  0.138016 &  0.133244  \\
$\mathbb{M}_\mathrm{ent}$ &  0.160556  & 0.146313  &  0.144865 &  0.136778  \\
$\mathbb{M}_\mathrm{avg\ ent}$ &  0.199574  & 0.120575  &  0.208142 &  0.131972  \\
$\mathbb{M}_{\mathrm{CP\ }\alpha=0.05}$ &  0.190427  & 0.138634  &  0.188075 &  0.153301  \\
$\mathbb{M}_{\mathrm{CP\ }\alpha=0.1}$ &  0.183588  & 0.134914  &  0.195179 &  0.155650  \\
$\mathbb{M}_{\mathrm{CP\ }\alpha=0.2}$ & -0.087108  &-0.126243  &  0.029448 &  0.070866  \\
\midrule
$\mathbb{M}_\mathrm{fail}^{\mathrm{ref}}$ &  0.185803  & 0.176365  &  0.170867 &  0.172466  \\
$\mathbb{M}_\mathrm{1^{st}\ layer}^{\mathrm{ref}}$ &  0.201608  & 0.192833  &  0.201257 &  0.184286  \\
$\mathbb{M}_\mathrm{1^{st}\ ckpt}^{\mathrm{ref}}$ &  0.201567  & 0.190652  &  0.198989 &  0.200628  \\
$\mathbb{M}_\mathrm{avg\ ckpt}^{\mathrm{ref}}$ &  0.186492  & 0.177996  &  0.173982 &  0.174868  \\
$\mathbb{M}_{\mathrm{avg\ ckpt\ }p}^{\mathrm{ref}}$ &  0.225674  & 0.189274  &  0.221395 &  0.188518  \\
\bottomrule
\end{tabular}


% hard labels, original
% \begin{tabular}{lrr}
% \toprule
%  & $\mathbb{H}_\mathrm{ent}$ & $\mathbb{H}_\mathrm{dis}$ \\
% \midrule
% $\mathbb{H}_\mathrm{ent}$ & 1.000000 & 1.000000 \\
% $\mathbb{H}_\mathrm{dis}$ & 1.000000 & 1.000000 \\
% $\mathbb{M}_\mathrm{dis}$ & 0.133244 &\\
% $\mathbb{M}_\mathrm{ent}$ & 0.136778 &\\
% $\mathbb{M}_\mathrm{avg\ ent}$ & 0.131972 &\\
% $\mathbb{M}_{\mathrm{CP\ }\alpha=0.05}^{+\mathrm{ref}}$ & 0.153301 &\\
% $\mathbb{M}_{\mathrm{CP\ }\alpha=0.1}^{+\mathrm{ref}}$ & 0.155650 &\\
% $\mathbb{M}_{\mathrm{CP\ }\alpha=0.2}^{+\mathrm{ref}}$ & 0.070866 &\\
% \midrule
% $\mathbb{M}_\mathrm{fail}^{+\mathrm{ref}}$ & 0.172466 &\\
% $\mathbb{M}_\mathrm{1^{st}\ layer}^{+\mathrm{ref}}$ & 0.184286 &\\
% $\mathbb{M}_\mathrm{1^{st}\ ckpt}^{+\mathrm{ref}}$ & 0.200628 &\\
% $\mathbb{M}_\mathrm{avg\ ckpt}^{+\mathrm{ref}}$ & 0.174868 &\\
% $\mathbb{M}_{\mathrm{avg\ ckpt\ }p}^{+\mathrm{ref}}$ & 0.188518 &\\
% \bottomrule
% \end{tabular}

% soft labels, original
% \begin{tabular}{lrr}
% \toprule
%  & $\mathbb{H}_\mathrm{ent}$ & $\mathbb{H}_\mathrm{dis}$ \\
% \midrule
% $\mathbb{H}_\mathrm{ent}$ & 1.000000 & 1.000000 \\
% $\mathbb{H}_\mathrm{dis}$ & 1.000000 & 1.000000 \\
% $\mathbb{M}_\mathrm{dis}$ & 0.138016 &\\
% $\mathbb{M}_\mathrm{ent}$ & 0.144865 &\\
% $\mathbb{M}_\mathrm{avg\ ent}$ & 0.208142 &\\
% $\mathbb{M}_{\mathrm{CP\ }\alpha=0.05}^{+\mathrm{ref}}$ & 0.188075 &\\
% $\mathbb{M}_{\mathrm{CP\ }\alpha=0.1}^{+\mathrm{ref}}$ & 0.195179 &\\
% $\mathbb{M}_{\mathrm{CP\ }\alpha=0.2}^{+\mathrm{ref}}$ & 0.029448 &\\
% \midrule
% $\mathbb{M}_\mathrm{fail}^{+\mathrm{ref}}$ & 0.170867 &\\
% $\mathbb{M}_\mathrm{1^{st}\ layer}^{+\mathrm{ref}}$ & 0.201257 &\\
% $\mathbb{M}_\mathrm{1^{st}\ ckpt}^{+\mathrm{ref}}$ & 0.198989 &\\
% $\mathbb{M}_\mathrm{avg\ ckpt}^{+\mathrm{ref}}$ & 0.173982 &\\
% $\mathbb{M}_{\mathrm{avg\ ckpt\ }p}^{+\mathrm{ref}}$ & 0.221395 &\\
% \bottomrule
% \end{tabular}

% hard, re-balanced
% \begin{tabular}{lrr}
% \toprule
%  & $\mathbb{H}_\mathrm{ent}$ & $\mathbb{H}_\mathrm{dis}$ \\
% \midrule
% $\mathbb{H}_\mathrm{ent}$ & 1.000000 & 1.000000 \\
% $\mathbb{H}_\mathrm{dis}$ & 1.000000 & 1.000000 \\
% $\mathbb{M}_\mathrm{dis}$ & 0.143457 &\\
% $\mathbb{M}_\mathrm{ent}$ & 0.146313 &\\
% $\mathbb{M}_\mathrm{avg\ ent}$ & 0.120575 &\\
% $\mathbb{M}_{\mathrm{CP\ }\alpha=0.05}^{+\mathrm{ref}}$ & 0.138634 &\\
% $\mathbb{M}_{\mathrm{CP\ }\alpha=0.1}^{+\mathrm{ref}}$ & 0.134914 &\\
% $\mathbb{M}_{\mathrm{CP\ }\alpha=0.2}^{+\mathrm{ref}}$ & -0.126243 & \\
% \midrule
% $\mathbb{M}_\mathrm{fail}^{+\mathrm{ref}}$ & 0.176365 &\\
% $\mathbb{M}_\mathrm{1^{st}\ layer}^{+\mathrm{ref}}$ & 0.192833 &\\
% $\mathbb{M}_\mathrm{1^{st}\ ckpt}^{+\mathrm{ref}}$ & 0.190652 &\\
% $\mathbb{M}_\mathrm{avg\ ckpt}^{+\mathrm{ref}}$ & 0.177996 &\\
% $\mathbb{M}_{\mathrm{avg\ ckpt\ }p}^{+\mathrm{ref}}$ & 0.189274 &\\
% \bottomrule
% \end{tabular}


% soft, re-balanced
% \begin{tabular}{lrr}
% \toprule
%  & $\mathbb{H}_\mathrm{ent}$ & $\mathbb{H}_\mathrm{dis}$ \\
% \midrule
% $\mathbb{H}_\mathrm{ent}$ & 1.000000 & 1.000000 \\
% $\mathbb{H}_\mathrm{dis}$ & 1.000000 & 1.000000 \\
% $\mathbb{M}_\mathrm{dis}$ & 0.155306 &\\
% $\mathbb{M}_\mathrm{ent}$ & 0.160556 &\\
% $\mathbb{M}_\mathrm{avg\ ent}$ & 0.199574 &\\
% $\mathbb{M}_{\mathrm{CP\ }\alpha=0.05}^{+\mathrm{ref}}$ & 0.190427 &\\
% $\mathbb{M}_{\mathrm{CP\ }\alpha=0.1}^{+\mathrm{ref}}$ & 0.183588 &\\
% $\mathbb{M}_{\mathrm{CP\ }\alpha=0.2}^{+\mathrm{ref}}$ & -0.087108 & \\
% \midrule
% $\mathbb{M}_\mathrm{fail}^{+\mathrm{ref}}$ & 0.185803 &\\
% $\mathbb{M}_\mathrm{1^{st}\ layer}^{+\mathrm{ref}}$ & 0.201608 &\\
% $\mathbb{M}_\mathrm{1^{st}\ ckpt}^{+\mathrm{ref}}$ & 0.201567 &\\
% $\mathbb{M}_\mathrm{avg\ ckpt}^{+\mathrm{ref}}$ & 0.186492 &\\
% $\mathbb{M}_{\mathrm{avg\ ckpt\ }p}^{+\mathrm{ref}}$ & 0.225674 &\\
% \bottomrule
% \end{tabular}

==> Tables/dynasent-results/spearman-vs-h-ent-bert.tex <==
\begin{tabular}{l  S[table-format=2.4] S[table-format=2.4] S[table-format=2.4] S[table-format=2.4] } %r rrr r rrrr} % <================================ p{6cm}
\toprule
 & \multicolumn{2}{c}{re-balanced} & \multicolumn{2}{c}{original} \\
 & {{soft}} & {{hard}} & {{soft}} & {{hard}} \\
\midrule
$\mathbb{M}_\mathrm{dis}$ &  0.067947 & 0.065404 & 0.069460  & 0.069930  \\
$\mathbb{M}_\mathrm{ent}$ &  0.070805 & 0.063082 & 0.071170  & 0.080061  \\
$\mathbb{M}_\mathrm{avg\ ent}$ &  0.139525 & 0.126554 & 0.141544  & 0.130062  \\
$\mathbb{M}_{\mathrm{CP\ }\alpha=0.05}$ & 0.122310 & 0.107492 & 0.127812  & 0.126454  \\
$\mathbb{M}_{\mathrm{CP\ }\alpha=0.1}$ & 0.117745 & 0.099780 & 0.129200  & 0.125054  \\
$\mathbb{M}_{\mathrm{CP\ }\alpha=0.2}$ & 0.109955 & 0.081290 & 0.124749  & 0.108697  \\
\midrule
$\mathbb{M}_\mathrm{fail}^{\mathrm{ref}}$ & 0.128621 & 0.115634 & 0.139867  & 0.142633  \\
$\mathbb{M}_\mathrm{1^{st}\ layer}^{\mathrm{ref}}$ & 0.131855 & 0.123511 & 0.123916  & 0.120525  \\
$\mathbb{M}_\mathrm{1^{st}\ ckpt}^{\mathrm{ref}}$ &  0.131310 & 0.113666 & 0.141114  & 0.143787  \\
$\mathbb{M}_\mathrm{avg\ ckpt}^{\mathrm{ref}}$ &  0.126832 & 0.113302 & 0.134444  & 0.137036  \\
$\mathbb{M}_{\mathrm{avg\ ckpt\ }p}^{\mathrm{ref}}$ &  0.150418 & 0.135961 & 0.162732 & 0.160526  \\
\bottomrule
\end{tabular}

% % labeltype = 'hard'
% % balanced = False

% \begin{tabular}{lrr}
% \toprule
%  & $\mathbb{H}_\mathrm{ent}$ & $\mathbb{H}_\mathrm{dis}$ \\
% \midrule
% $\mathbb{M}_\mathrm{dis}$ & 0.069930 & \\
% $\mathbb{M}_\mathrm{ent}$ & 0.080061 & \\
% $\mathbb{M}_\mathrm{avg\ ent}$ & 0.130062 & \\
% $\mathbb{M}_{\mathrm{CP\ }\alpha=0.05}$ & 0.126454 & \\
% $\mathbb{M}_{\mathrm{CP\ }\alpha=0.1}$ & 0.125054 & \\
% $\mathbb{M}_{\mathrm{CP\ }\alpha=0.2}$ & 0.108697 & \\
% \midrule
% $\mathbb{M}_\mathrm{fail}^{\mathrm{ref}}$ & 0.142633 & \\
% $\mathbb{M}_\mathrm{1^{st}\ layer}^{\mathrm{ref}}$ & 0.120525 & \\
% $\mathbb{M}_\mathrm{1^{st}\ ckpt}^{\mathrm{ref}}$ & 0.143787 & \\
% $\mathbb{M}_\mathrm{avg\ ckpt}^{\mathrm{ref}}$ & 0.137036 & \\
% $\mathbb{M}_{\mathrm{avg\ ckpt\ }p}^{\mathrm{ref}}$ & 0.160526 & \\
% \bottomrule
% \end{tabular}



% % labeltype = 'soft'
% % balanced = False

% \begin{tabular}{lrr}
% \toprule
%  & $\mathbb{H}_\mathrm{ent}$ & $\mathbb{H}_\mathrm{dis}$ \\
% \midrule
% $\mathbb{M}_\mathrm{dis}$ & 0.069460 & \\
% $\mathbb{M}_\mathrm{ent}$ & 0.071170 & \\
% $\mathbb{M}_\mathrm{avg\ ent}$ & 0.141544 & \\
% $\mathbb{M}_{\mathrm{CP\ }\alpha=0.05}$ & 0.127812 & \\
% $\mathbb{M}_{\mathrm{CP\ }\alpha=0.1}$ & 0.129200 & \\
% $\mathbb{M}_{\mathrm{CP\ }\alpha=0.2}$ & 0.124749 & \\
% \midrule
% $\mathbb{M}_\mathrm{fail}^{\mathrm{ref}}$ & 0.139867 & \\
% $\mathbb{M}_\mathrm{1^{st}\ layer}^{\mathrm{ref}}$ & 0.123916 & \\
% $\mathbb{M}_\mathrm{1^{st}\ ckpt}^{\mathrm{ref}}$ & 0.141114 & \\
% $\mathbb{M}_\mathrm{avg\ ckpt}^{\mathrm{ref}}$ & 0.134444 & \\
% $\mathbb{M}_{\mathrm{avg\ ckpt\ }p}^{\mathrm{ref}}$ & 0.162732 & \\
% \bottomrule
% \end{tabular}

% % labeltype = 'hard'
% % balanced = True

% \begin{tabular}{lrr}
% \toprule
%  & $\mathbb{H}_\mathrm{ent}$ & $\mathbb{H}_\mathrm{dis}$ \\
% \midrule
% $\mathbb{M}_\mathrm{dis}$ & 0.065404 &  \\
% $\mathbb{M}_\mathrm{ent}$ & 0.063082 &  \\
% $\mathbb{M}_\mathrm{avg\ ent}$ & 0.126554 &  \\
% $\mathbb{M}_{\mathrm{CP\ }\alpha=0.05}$ & 0.107492 &  \\
% $\mathbb{M}_{\mathrm{CP\ }\alpha=0.1}$ & 0.099780 &  \\
% $\mathbb{M}_{\mathrm{CP\ }\alpha=0.2}$ & 0.081290 &  \\
% \midrule
% $\mathbb{M}_\mathrm{fail}^{\mathrm{ref}}$ & 0.115634 &  \\
% $\mathbb{M}_\mathrm{1^{st}\ layer}^{\mathrm{ref}}$ & 0.123511 &  \\
% $\mathbb{M}_\mathrm{1^{st}\ ckpt}^{\mathrm{ref}}$ & 0.113666 &  \\
% $\mathbb{M}_\mathrm{avg\ ckpt}^{\mathrm{ref}}$ & 0.113302 &  \\
% $\mathbb{M}_{\mathrm{avg\ ckpt\ }p}^{\mathrm{ref}}$ & 0.135961 &  \\
% \bottomrule
% \end{tabular}


% % labeltype = 'soft'
% % balanced = True
% \begin{tabular}{lrr}
% \toprule
%  & $\mathbb{H}_\mathrm{ent}$ & $\mathbb{H}_\mathrm{dis}$ \\
% \midrule
% $\mathbb{M}_\mathrm{dis}$ & 0.067947 &  \\
% $\mathbb{M}_\mathrm{ent}$ & 0.070805 &  \\
% $\mathbb{M}_\mathrm{avg\ ent}$ & 0.139525 &  \\
% $\mathbb{M}_{\mathrm{CP\ }\alpha=0.05}^{+\mathrm{ref}}$ & 0.122310 &  \\
% $\mathbb{M}_{\mathrm{CP\ }\alpha=0.1}^{+\mathrm{ref}}$ & 0.117745 &  \\
% $\mathbb{M}_{\mathrm{CP\ }\alpha=0.2}^{+\mathrm{ref}}$ & 0.109955 &  \\
% \midrule
% $\mathbb{M}_\mathrm{fail}^{+\mathrm{ref}}$ & 0.128621 &  \\
% $\mathbb{M}_\mathrm{1^{st}\ layer}^{+\mathrm{ref}}$ & 0.131855 &  \\
% $\mathbb{M}_\mathrm{1^{st}\ ckpt}^{+\mathrm{ref}}$ & 0.131310 &  \\
% $\mathbb{M}_\mathrm{avg\ ckpt}^{+\mathrm{ref}}$ & 0.126832 &  \\
% $\mathbb{M}_{\mathrm{avg\ ckpt\ }p}^{+\mathrm{ref}}$ & 0.150418 &  \\
% \bottomrule
% \end{tabular}



==> Tables/dynasent-results/spearmans/dynasent-balanced-hard.tex <==
\begin{tabular}{l  S[table-format=1.4] S[table-format=1.4] } %r rrr r rrrr} % <================================ p{6cm}
\toprule
 & $\mathbb{H}_\mathrm{ent}$ & $\mathbb{H}_\mathrm{dis}$ \\
\midrule
$\mathbb{M}_\mathrm{dis}$ & 0.089156 & 0.089156 \\
$\mathbb{M}_\mathrm{ent}$ & 0.098924 & 0.098924 \\
$\mathbb{M}_\mathrm{avg\ ent}$ & 0.085084 & 0.085084 \\
$\mathbb{M}_{\mathrm{CP\ }\alpha=0.05}$ & 0.087629 & 0.087629 \\
$\mathbb{M}_{\mathrm{CP\ }\alpha=0.1}$ & 0.083157 & 0.083157 \\
$\mathbb{M}_{\mathrm{CP\ }\alpha=0.2}$ & 0.074868 & 0.074868 \\
\midrule
$\mathbb{M}_\mathrm{fail}^{\mathrm{ref}}$ & 0.141376 & 0.141376 \\
$\mathbb{M}_\mathrm{1^{st}\ layer}^{\mathrm{ref}}$ & 0.132864 & 0.132864 \\
$\mathbb{M}_\mathrm{1^{st}\ ckpt}^{\mathrm{ref}}$ & 0.152962 & 0.152962 \\
$\mathbb{M}_\mathrm{avg\ ckpt}^{\mathrm{ref}}$ & 0.148958 & 0.148958 \\
$\mathbb{M}_{\mathrm{avg\ ckpt\ }p}^{\mathrm{ref}}$ & 0.158176 & 0.158176 \\
\bottomrule
\end{tabular}

==> Tables/dynasent-results/spearmans/dynasent-balanced-soft.tex <==
\begin{tabular}{l  S[table-format=1.4] S[table-format=1.4] } %r rrr r rrrr} % <================================ p{6cm}
\toprule
 & $\mathbb{H}_\mathrm{ent}$ & $\mathbb{H}_\mathrm{dis}$ \\
\midrule
$\mathbb{M}_\mathrm{dis}$ & 0.094977 & 0.094977 \\
$\mathbb{M}_\mathrm{ent}$ & 0.108877 & 0.108877 \\
$\mathbb{M}_\mathrm{avg\ ent}$ & 0.150654 & 0.150654 \\
$\mathbb{M}_{\mathrm{CP\ }\alpha=0.05}$ & 0.138518 & 0.138518 \\
$\mathbb{M}_{\mathrm{CP\ }\alpha=0.1}$ & 0.148467 & 0.148467 \\
$\mathbb{M}_{\mathrm{CP\ }\alpha=0.2}$ & 0.124065 & 0.124065 \\
\midrule
$\mathbb{M}_\mathrm{fail}^{\mathrm{ref}}$ & 0.148555 & 0.148555 \\
$\mathbb{M}_\mathrm{1^{st}\ layer}^{\mathrm{ref}}$ & 0.137065 & 0.137065 \\
$\mathbb{M}_\mathrm{1^{st}\ ckpt}^{\mathrm{ref}}$ & 0.164345 & 0.164345 \\
$\mathbb{M}_\mathrm{avg\ ckpt}^{\mathrm{ref}}$ & 0.155180 & 0.155180 \\
$\mathbb{M}_{\mathrm{avg\ ckpt\ }p}^{\mathrm{ref}}$ & 0.179580 & 0.179580 \\
\bottomrule
\end{tabular}

==> Tables/dynasent-results/spearmans/dynasent-unbalanced-hard.tex <==
\begin{tabular}{l  S[table-format=1.4] S[table-format=1.4] } %r rrr r rrrr} % <================================ p{6cm}
\toprule
 & $\mathbb{H}_\mathrm{ent}$ & $\mathbb{H}_\mathrm{dis}$ \\
\midrule
$\mathbb{M}_\mathrm{dis}$ & 0.115266 & 0.115266 \\
$\mathbb{M}_\mathrm{ent}$ & 0.122671 & 0.122671 \\
$\mathbb{M}_\mathrm{avg\ ent}$ & 0.091493 & 0.091493 \\
$\mathbb{M}_{\mathrm{CP\ }\alpha=0.05}$ & 0.113891 & 0.113891 \\
$\mathbb{M}_{\mathrm{CP\ }\alpha=0.1}$ & 0.102674 & 0.102674 \\
$\mathbb{M}_{\mathrm{CP\ }\alpha=0.2}$ & 0.094476 & 0.094476 \\
\midrule
$\mathbb{M}_\mathrm{fail}^{\mathrm{ref}}$ & 0.163033 & 0.163033 \\
$\mathbb{M}_\mathrm{1^{st}\ layer}^{\mathrm{ref}}$ & 0.165423 & 0.165423 \\
$\mathbb{M}_\mathrm{1^{st}\ ckpt}^{\mathrm{ref}}$ & 0.182930 & 0.182930 \\
$\mathbb{M}_\mathrm{avg\ ckpt}^{\mathrm{ref}}$ & 0.164045 & 0.164045 \\
$\mathbb{M}_{\mathrm{avg\ ckpt\ }p}^{\mathrm{ref}}$ & 0.177427 & 0.177427 \\
\bottomrule
\end{tabular}

==> Tables/dynasent-results/spearmans/dynasent-unbalanced-soft.tex <==
\begin{tabular}{l  S[table-format=1.4] S[table-format=1.4] } %r rrr r rrrr} % <================================ p{6cm}
\toprule
 & $\mathbb{H}_\mathrm{ent}$ & $\mathbb{H}_\mathrm{dis}$ \\
\midrule
$\mathbb{M}_\mathrm{dis}$ & 0.112997 & 0.112997 \\
$\mathbb{M}_\mathrm{ent}$ & 0.122802 & 0.122802 \\
$\mathbb{M}_\mathrm{avg\ ent}$ & 0.160867 & 0.160867 \\
$\mathbb{M}_{\mathrm{CP\ }\alpha=0.05}$ & 0.132735 & 0.132735 \\
$\mathbb{M}_{\mathrm{CP\ }\alpha=0.1}$ & 0.139800 & 0.139800 \\
$\mathbb{M}_{\mathrm{CP\ }\alpha=0.2}$ & 0.151360 & 0.151360 \\
\midrule
$\mathbb{M}_\mathrm{fail}^{\mathrm{ref}}$ & 0.165565 & 0.165565 \\
$\mathbb{M}_\mathrm{1^{st}\ layer}^{\mathrm{ref}}$ & 0.186068 & 0.186068 \\
$\mathbb{M}_\mathrm{1^{st}\ ckpt}^{\mathrm{ref}}$ & 0.188283 & 0.188283 \\
$\mathbb{M}_\mathrm{avg\ ckpt}^{\mathrm{ref}}$ & 0.166829 & 0.166829 \\
$\mathbb{M}_{\mathrm{avg\ ckpt\ }p}^{\mathrm{ref}}$ & 0.191361 & 0.191361 \\
\bottomrule
\end{tabular}

==> Tables/mnli-results/mnli-spearman-1b-vs-humans.tex <==
\begin{tabular}{l  S[table-format=2.4] S[table-format=2.4] } %r rrr r rrrr} % <================================ p{6cm}
\toprule
 & $\mathbb{H}_\mathrm{ent}$ & $\mathbb{H}_\mathrm{dis}$ \\
\midrule
% $\mathbb{H}_\mathrm{ent}$ & 1.000000 & 0.896358 \\
% $\mathbb{H}_\mathrm{dis}$ & 0.896358 & 1.000000 \\
$\mathbb{M}_\mathrm{dis}$ & 0.141883 & 0.107431 \\
$\mathbb{M}_\mathrm{ent}$ & 0.158733 & 0.120148 \\
$\mathbb{M}_\mathrm{avg\ ent}$ & 0.132883 & 0.109529 \\
$\mathbb{M}_{\mathrm{CP\ }\alpha=0.05}$ & 0.078811 & 0.042506 \\
$\mathbb{M}_{\mathrm{CP\ }\alpha=0.1}$ & 0.179797 & 0.116383 \\
$\mathbb{M}_{\mathrm{CP\ }\alpha=0.2}$ & 0.158052 & 0.093621 \\
\midrule
$\mathbb{M}_\mathrm{fail}^{\mathrm{ref}}$ & 0.172586 & 0.224618 \\
$\mathbb{M}_\mathrm{1^{st}\ layer}^{\mathrm{ref}}$ & 0.204044 & 0.251401 \\
$\mathbb{M}_\mathrm{1^{st}\ ckpt}^{\mathrm{ref}}$ & 0.182928 & 0.230737 \\
$\mathbb{M}_\mathrm{avg\ ckpt}^{\mathrm{ref}}$ & 0.176423 & 0.226072 \\
$\mathbb{M}_{\mathrm{avg\ ckpt\ }p}^{\mathrm{ref}}$ & 0.181264 & 0.230670 \\
\bottomrule
\end{tabular}

==> Tables/mnli-results/mnli-spearman-bert-vs-humans.tex <==
\begin{tabular}{l  S[table-format=2.4] S[table-format=2.4] } %r rrr r rrrr} % <================================ p{6cm}
\toprule
 & $\mathbb{H}_\mathrm{ent}$ & $\mathbb{H}_\mathrm{dis}$ \\
\midrule
% $\mathbb{H}_\mathrm{ent}$ & 1.000000 & 0.896358 \\
% $\mathbb{H}_\mathrm{dis}$ & 0.896358 & 1.000000 \\
$\mathbb{M}_\mathrm{dis}$ & -0.002232 & -0.004482 \\
$\mathbb{M}_\mathrm{ent}$ & 0.002331 & -0.001140 \\
$\mathbb{M}_\mathrm{avg\ ent}$ & -0.007652 & -0.015789 \\
$\mathbb{M}_{\mathrm{CP\ }\alpha=0.05}$ & 0.010060 & -0.008535 \\
$\mathbb{M}_{\mathrm{CP\ }\alpha=0.1}$ & -0.007260 & -0.017336 \\
$\mathbb{M}_{\mathrm{CP\ }\alpha=0.2}$ & -0.018384 & -0.023108 \\
\midrule
$\mathbb{M}_\mathrm{fail}^{\mathrm{ref}}$ & 0.117376 & 0.150791 \\
$\mathbb{M}_\mathrm{1^{st}\ layer}^{\mathrm{ref}}$ & 0.068166 & 0.096622 \\
$\mathbb{M}_\mathrm{1^{st}\ ckpt}^{\mathrm{ref}}$ & 0.113171 & 0.147928 \\
$\mathbb{M}_\mathrm{avg\ ckpt}^{\mathrm{ref}}$ & 0.116766 & 0.149847 \\
$\mathbb{M}_{\mathrm{avg\ ckpt\ }p}^{\mathrm{ref}}$ & 0.109385 & 0.143412 \\
\bottomrule
\end{tabular}

==> Tables/models.tex <==
\begin{table}[th]
    \centering
\resizebox{\columnwidth}{!}{
\begin{tabular}{ >{\tt}l r c}
\toprule
model\_name & $N_{param}$ & model\_id \\
\midrule
bert\_uncased\_L-2\_H-128\_A-2 & 4,385,920 & $\theta_1$ \\
bert\_uncased\_L-4\_H-128\_A-2 & 4,782,464 & $\theta_2$ \\
bert\_uncased\_L-6\_H-128\_A-2 & 5,179,008 & $\theta_3$ \\
bert\_uncased\_L-8\_H-128\_A-2 & 5,575,552 & $\theta_4$ \\
bert\_uncased\_L-10\_H-128\_A-2 & 5,972,096 & $\theta_5$ \\
bert\_uncased\_L-12\_H-128\_A-2 & 6,368,640 & $\theta_6$ \\
bert\_uncased\_L-2\_H-256\_A-4 & 9,591,040 & $\theta_7$ \\
bert\_uncased\_L-4\_H-256\_A-4 & 11,170,560 & $\theta_8$ \\
bert\_uncased\_L-6\_H-256\_A-4 & 12,750,080 & $\theta_9$ \\
bert\_uncased\_L-8\_H-256\_A-4 & 14,329,600 & $\theta_{10}$ \\
bert\_uncased\_L-10\_H-256\_A-4 & 15,909,120 & $\theta_{11}$ \\
bert\_uncased\_L-12\_H-256\_A-4 & 17,488,640 & $\theta_{12}$ \\
bert\_uncased\_L-2\_H-512\_A-8 & 22,458,880 & $\theta_{13}$ \\
bert\_uncased\_L-4\_H-512\_A-8 & 28,763,648 & $\theta_{14}$ \\
bert\_uncased\_L-6\_H-512\_A-8 & 35,068,416 & $\theta_{15}$ \\
bert\_uncased\_L-2\_H-768\_A-12 & 38,603,520 & $\theta_{16}$ \\
bert\_uncased\_L-8\_H-512\_A-8 & 41,373,184 & $\theta_{17}$ \\
bert\_uncased\_L-10\_H-512\_A-8 & 47,677,952 & $\theta_{18}$ \\
bert\_uncased\_L-4\_H-768\_A-12 & 52,779,264 & $\theta_{19}$ \\
bert\_uncased\_L-12\_H-512\_A-8 & 53,982,720 & $\theta_{20}$ \\
bert\_uncased\_L-6\_H-768\_A-12 & 66,955,008 & $\theta_{21}$ \\
bert\_uncased\_L-8\_H-768\_A-12 & 81,130,752 & $\theta_{22}$ \\
bert\_uncased\_L-10\_H-768\_A-12 & 95,306,496 & $\theta_{23}$ \\
bert\_uncased\_L-12\_H-768\_A-12 & 109,482,240 & $\theta_{24}$ \\
\midrule

EleutherAI/pythia-1b-deduped & 908,759,040 & $\theta_{25}$ \\
bigscience/bloom-1b1 & 1,065,314,304 & $\theta_{26}$ \\
allenai/OLMo-1B-hf & 1,176,764,416 & $\theta_{27}$ \\
meta-llama/Llama-3.2-1B & 1,235,814,400 & $\theta_{28}$ \\
tiiuae/falcon-rw-1b & 1,311,625,216 & $\theta_{29}$ \\

\bottomrule
\end{tabular}}
    \caption{model complexity}
    \label{tab:complexmodels}
\end{table}

==> Tables/r2-models.tex <==
\begin{table}[ht!]
\centering
    \begin{subfigure}[b]{0.95\columnwidth}
        \centering
        \resizebox{\textwidth}{!}{
\begin{tabular}{l  S[table-format=1.4] S[table-format=1.4]  S[table-format=1.4] S[table-format=1.4] } %r rrr r rrrr} % <================================ p{6cm}
\toprule
{} &  $\mathbb{M}_\mathrm{fail}^{+\mathrm{ref}}$ & $\mathbb{M}_\mathrm{avg\ ckpt}^{+\mathrm{ref}}$ & $\mathbb{M}_\mathrm{1^{st}\ ckpt}^{+\mathrm{ref}}$ & $\mathbb{M}_\mathrm{1^{st}\ layer}^{+\mathrm{ref}}$ \\ \midrule
$\mathbb{M}_\mathrm{dis}^{\neg\mathrm{ref}}$ & 0.17588598651476195 & 0.21381786790938095 & 0.35649990339441595 & 0.19440046850418435\\
$\mathbb{M}_\mathrm{avg\ ent}^{\neg\mathrm{ref}}$ & 0.1782489981245251 & 0.22729472265941164 & 0.3982724719893981 & 0.19696870432653812\\
$\mathbb{M}_\mathrm{ent}^{\neg\mathrm{ref}}$ & 0.19773962539055912 & 0.24253367571639584 & 0.4077789195636078 & 0.21881173192547088\\\bottomrule
\end{tabular}
}
\caption{<1B models}
\label{tab:r2-models-bert}
    \end{subfigure}    

\vspace{0.1cm}
    
    \begin{subfigure}[b]{0.95\columnwidth}
        \centering
        \resizebox{\textwidth}{!}{
\centering
\begin{tabular}{l  S[table-format=1.4] S[table-format=1.4]  S[table-format=1.4] S[table-format=1.4] } %rrrrrrr}
\toprule
{} & $\mathbb{M}_\mathrm{fail}^{+\mathrm{ref}}$ & $\mathbb{M}_\mathrm{avg\ ckpt}^{+\mathrm{ref}}$ & $\mathbb{M}_\mathrm{1^{st}\ ckpt}^{+\mathrm{ref}}$ & $\mathbb{M}_\mathrm{1^{st}\ layer}^{+\mathrm{ref}}$ \\
\midrule
$\mathbb{M}_\mathrm{dis}^{\neg\mathrm{ref}}$ & 0.16413265457282322 & 0.2459899273918863 & 0.3361874018157971 & 0.17701440036916938\\
$\mathbb{M}_\mathrm{avg\ ent}^{\neg\mathrm{ref}}$ & 0.19155081162607945 & 0.3158621785630321 & 0.4321987166946284 & 0.21743121881888716\\
$\mathbb{M}_\mathrm{ent}^{\neg\mathrm{ref}}$ & 0.17996877177974802 & 0.2715791550947587 & 0.37888784176142787 & 0.19761162079599937\\
\bottomrule
\end{tabular}
        }
\caption{1B models}
\label{tab:r2-models-1b}
    \end{subfigure}    
\caption{Proportion of explained variance ($R^2$) of linear regressions predicting a reference-dependent indicator from a reference-free indicator}
\label{tab:r2-models}
\end{table}
%\vspace{-2cm}

==> Tables/shap-feature-importance.tex <==


\begin{table}[ht]
    
    \begin{subfigure}[b]{\columnwidth}
    \centering
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{l l S[table-format=1.4] S[table-format=1.4] S[table-format=1.4] S[table-format=1.4]  S[table-format=1.4]}
        \toprule
         & & \multicolumn{5}{c}{\textbf{Predicted value}} \\
         & & {$\mathbb{M}_\mathrm{fail}$} & {$\mathbb{M}_\mathrm{avg\ ent}$} & {$\mathbb{M}_\mathrm{avg\ ckpt}^{+\mathrm{ref}}$} & {$\mathbb{M}_\mathrm{1^{st}\ ckpt}^{+\mathrm{ref}}$} & {$\mathbb{M}_\mathrm{1^{st}\ layer}^{+\mathrm{ref}}$} \\  \midrule
         \multirow{3}{*}{\rotatebox{90}{\textbf{Feature}}} 
& $\mathbb{H}_\mathrm{ent}$ & 0.261068 & 0.201172 & 0.310571 & 0.299462 & 0.251123 \\
& $\log_{10}$ params & 0.029067 & 0.091583 & 0.033300 & 0.043741 & 0.169547 \\
& Training split & 0.001502 & 0.031730 & 0.002236 & 0.001821 & 0.039451 \\ \bottomrule
    \end{tabular}}
    \caption{\label{tab:shap estimates:without data}Without categorical variable for datapoints}
    \end{subfigure}
    
    \begin{subfigure}[b]{\columnwidth}
    \centering
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{l l S[table-format=1.4] S[table-format=1.4] S[table-format=1.4] S[table-format=1.4]  S[table-format=1.4]}
        \toprule
         & & \multicolumn{5}{c}{\textbf{Predicted value}} \\
         & & {$\mathbb{M}_\mathrm{fail}$} & {$\mathbb{M}_\mathrm{avg\ ent}$} & {$\mathbb{M}_\mathrm{avg\ ckpt}^{+\mathrm{ref}}$} & {$\mathbb{M}_\mathrm{1^{st}\ ckpt}^{+\mathrm{ref}}$} & {$\mathbb{M}_\mathrm{1^{st}\ layer}^{+\mathrm{ref}}$} \\  \midrule
         \multirow{4}{*}{\rotatebox{90}{\textbf{Feature}}} 
& $\mathbb{H}_\mathrm{ent}$ & 0.071904 & 0.042620 & 0.081924 & 0.076632 & 0.068104 \\
& $\log_{10}$ params & 0.026468 & 0.073430 & 0.032394 & 0.040444 & 0.149773 \\
& Training split & 0.060880 & 0.074350 & 0.051965 & 0.061884 & 0.077918 \\
& Datapoint & 0.577426 & 0.564823 & 0.701543 & 0.650862 & 0.557907 \\ \bottomrule
    \end{tabular}}
    \caption{\label{tab:shap estimates:with data}With categorical variable for datapoints}
    \end{subfigure}
    
    
    \caption{Mean absolute SHAP estimates of feature importance (1B models)}
    \label{tab:shap estimates}
\end{table}

==> background.tex <==
Our study falls in the intersection of data uncertainty and complexity in NLP, particularly in relation to annotator disagreement, data complexity, and the metrics commonly used to evaluate these phenomena. \citep{jiang-marneffe-2022-investigating, Uma2021, lorena2019howcomplex, baan2023uncertainty}.

%\paragraph{Data Uncertainty} 
We borrow the definition of \textbf{data uncertainty} (aka. aleatoric uncertainty) from \citet{hu2023uncertainty}, which refers to this type of uncertainty inherent in data due to its randomness or noise. This type of uncertainty is irreducible, meaning it cannot be eliminated through model improvements or tuning \citep{KIUREGHIAN2009105,kendall2017uncertainties,Hüllermeier2021}.
It can arise from a variety of sources, such as noisy
observations, overlapping classes, ground truth errors or inherent randomness. % or other factors that are not entirely predictable.
% In the Bayesian literature, uncertainty associated to a data sample is estimated using the \textit{predictive distribution} \citep[e.g.,][]{murphy2022MLbook}:
% \begin{equation}
%     P(y^\ast | x) = \int P(y^\ast |x, \theta) P(\theta|D) d\theta,
%     \label{eq:total_unc}
% \end{equation}
% where $d\theta$ denotes the model space and is intractable. In practice, we sample countable set of models $\theta$, each differing in pretraining and fine-tuning data, algorithmic and architectural designs, or parameter counts to approximate the entire model space. 

\textbf{Annotator disagreement} has been highlighted as a fundamental characteristic of linguistic data, emphasizing that dissensus arises primarily from the inherent ambiguity and richness of language, rather than from annotation noise alone \citep{plank-etal-2014-linguistically, Aroyo2015, pavlick-kwiatkowski-2019-inherent,fornaciari-etal-2021-beyond}. This phenomenon often correlates with \textbf{label uncertainty}, reflecting the difficulty of assigning a single definitive label to a datapoint. 
Numerous works demonstrate that high-disagreement examples contain valuable signals for classifiers \citep{basile-etal-2021-need, PalomakiRT18}. 
However, equating annotator disagreement with data complexity requires caution. While some approaches prioritize annotating uncertain examples --- often using label distribution entropy as a proxy \citep{zhang-etal-2022-survey, baumler-etal-2023-examples} --- this risks oversimplifying the issue. Label uncertainty reflects only one aspect of linguistic challenges and conflating it with broader data complexity may obscure nuances of human interpretation and model behavior.

\textbf{Data complexity} or data difficulty in NLP, refers to the characteristic of a data sample that can cause the latent representation to be too close to the decision boundary, making classification difficult. This can occur when the data point has a low-entropy class-wise distribution or, conversely, when it exhibits a high-entropy class-wise distribution. Data complexity encompasses various facets such as semantic indeterminacy, class overlap, and task-specific challenges,  making certain examples inherently harder for models to process \citep{plank-2022-problem,jiang-marneffe-2022-investigating}. 
%In \cref{eq:total_unc}, $P(y^\ast |x, \theta)$ represents the aleatoric uncertainty, which arises from the characteristics of $x$---specifically, the inherent ambiguity or noise in the language data.

While some foundational work focuses on image processing, works such as that of \citet{Peterson_2019_ICCV} --- which provides a framework for understanding label uncertainty caused by overlapping class boundaries --- are directly applicable to NLP tasks, where similar challenges are prevalent. Metrics for \textbf{evaluating data uncertainty and complexity}, including model confidence (e.g., probability of the predicted class), entropy of predicted probabilities, and calibrating the confidence to better align with performance offer insights into these phenomena \citep[e.g.,][]{geng-etal-2024-survey,ZHOU2022449,Xiao_Wang_2019}. Training dynamics, such as early classification success or the shape of the loss curve, further reveal the relative difficulty of datapoints \citep{swayamdipta-etal-2020-dataset,toneva2019Forgetting,baldock2021deep}. %PREVIOUSLY: For instance, measuring how early in the training process a model correctly classifies an example indicates how "easy" that data point is for the model, and analyzing the trajectory of loss curve reveals that examples with steep, quickly stabilizing loss curves are generally considered less complex \citep{swayamdipta-etal-2020-dataset, toneva2019Forgetting}.
While these metrics offer indirect signals to analyze the challenges of data complexity, they may not provide a nuanced perspective on the interplay between annotator disagreement and model uncertainty. 

To that end, it is worth stressing that human label variation and data complexity are often assumed to have overlapping causes. 
Whether these root causes are called overlapping classes \citep{990132,Peterson_2019_ICCV,lorena2019howcomplex}, absence of a single ground truth \citep{Aroyo2015,baan-etal-2022-stop}, or linguistic ambiguity due to semantic and social factors \citep{plank-2022-problem}, prior literature tends to agree despite differences in terminology that datapoints can be inherently more or less ambiguous, that annotators can be more or less accurate, and that these factors are responsible for the variation observed in human label variation, example difficulty and data uncertainty.%
% The view that label variation is tantamount to noise has been disproven by and large \citep[e.g.,][]{Aroyo2015},
% and modern accounts (esp. \citealp{plank-2022-problem}) rather stress that label variation arises from linguistic difficulty and linguistic ambiguity due to social or semantic factors, which is reminiscent of concerns regarding overlapping classes and the shape of decision boundaries from the data complexity literature \citep[e.g.,][]{990132,Peterson_2019_ICCV,lorena2019howcomplex}.
% \footnote{
%    Other root causes have been posited, in particular, outliers and label imbalances, \citep[e.g.,][]{990132} or out-of-domain distributions \citep[e.g.,][]{Gawlikowski2023}. %; the latter two can be controlled for by focusing on in-domain evaluation and well-balanced datasets.
%    As such, we focus on in-domain predictions and balanced training data.
% }
% In short, there is ample reason to consider that label variation, data complexity and data uncertainty are related phenomena with common underlying causes--- which therefore begs the question of whether model-centric metrics can %are well suited to 
% capture inherently subjective linguistic factors.
%As we show below, model-based metrics in fact often lead to diverging assessments of data complexity and alignment with annotator dissensus.
%In this paper, we contend that annotator disagreement directly reflects the inherent subjectivity of language interpretation, a dimension often overlooked by model-centric metrics like entropy.  We find that model behavior differences stem more from parameter counts than pretraining or fine-tuning, revealing how these metrics can lead to diverging assessments about data complexity and its alignment with annotator disagreement.    
 
%\citep{baan-etal-2022-stop}
%\citep{geng-etal-2024-survey}: https://aclanthology.org/2024.naacl-long.366.pdf
%a survey on uncertainty \& callibration in LLMs

%TODO insert barbara plank here

%TODO insert de marneffe here, specifically https://aclanthology.org/2022.tacl-1.78/ https://aclanthology.org/2021.naacl-main.390/

%https://www.sciencedirect.com/topics/engineering/aleatoric-uncertainty
%https://link.springer.com/article/10.1007/s10994-021-05946-3
%https://arxiv.org/pdf/2204.09308
%https://arxiv.org/abs/2406.15627

%https://aclanthology.org/2024.emnlp-main.443/
%https://aclanthology.org/2024.emnlp-main.181/
%https://aclanthology.org/2023.eacl-main.130/

%https://ojs.aaai.org/index.php/AAAI/article/view/4719

%https://arxiv.org/abs/2402.19460

%https://www.sciencedirect.com/science/article/abs/pii/S0957417413001413r

%\citep{kadasi-singh-2023-unveiling}

%Several works have explored uncertainty and found out that if we assume models to perform a certain way, it implies that we are assuming a behavior of the data set now. if the data inherent some noise gets it away from our assumed probability distribution, then the model will have difficulty in performing the downstream task.




% \paragraph{Comparison across different agents}
% Agents can be either human and machine (models). If we want to compare a skill between two groups $G_1$ and $G_2$, where $G_i$ denotes ith group for generality, in order for not re-invent the wheel we should consider the following: (a) In context of the skill, how does the prior i.e. the knowledge about the world or the training dataset in the two groups differ. (b) If group members of any group, say $G_1$ have the same prior they would tend to show same behavior. We can test it by sub-dividving the group $G_1$ into $G_{1,1}$ and $G_{1,2}$ and test for the same skill.
% Estimating the behavior of a group (wrt to a problem or another group) is non trivial when we do not have a knowledge or control over the prior the group was exposed to. So, $G_{1,1}$ and $G_{1,2}$ and more likely to be aligned if the entire $G_1$ was exposed to the same prior (training data). And, $G_1$ and $G_2$ are likely to have a different understanding or non-alignment for any skill or problem that we test them upon. 

\textcolor{red}{
In short, there is ample reason to consider that label variation, data complexity and data uncertainty are related phenomena with common underlying causes. 
Indeed, this is the position of \citet{Lalor2018-ft}, who look at item response theory data in humans and the probability mass assigned by models, and highlight a tendency of the two to align. This point of view is also prevalent in active learning \citep[e.g.,][]{hachey-etal-2005-investigating}, but also attested less directly in settings focusing on data quality \citep[e.g.,][]{jamison-gurevych-2015-noise}.
This link between data complexity and human label variation has also been presented on an anecdotal level, especially in works looking to understand causes for data complexity \citep{swayamdipta-etal-2020-dataset,baldock2021deep,rajpurkar-etal-2018-know}.
% We can list empirical studies making this claim \citet{Lalor2018-ft} look at item response theory data in humans and the probability mass assigned by models, and highlight a tendency of the two to align. This point of view is especially prevalent in active learning, e.g. \citet{hachey-etal-2005-investigating}, but also attested less directly in settings focusing on data quality, e.g. \citet{jamison-gurevych-2015-noise}.
%We can also cite works where this relationship is presented on an anecdotal level, e.g. \citet{swayamdipta-etal-2020-dataset} and \citet{baldock2021deep} which we already mentioned, but also \citet{rajpurkar-etal-2018-know}.
This perspective has also been employed as a working hypothesis, e.g. \citet{pmlr-v80-weinshall18a} who assume that knowledge distillation from a model can play the same role as humans in active learning scenarios, or \citet{beigman-beigman-klebanov-2009-learning} who propose to replace annotator-based disagreement assessment with classifier proxies.
This is often (though not always) combined with modeling work to better capture human variation (as in \citealp{reidsma-carletta-2008-squibs}) or discussions of the limitations of this working hypothesis (as in \citeauthor{beigman-beigman-klebanov-2009-learning}).
% We find groups of work who employ this perspective as a working hypothesis, e.g. \citet{pmlr-v80-weinshall18a} who assume that knowledge distillation from a model can play the same role as humans in active learning scenarios, or \citet{beigman-beigman-klebanov-2009-learning} who propose to replace annotator-based disagreement assessment with classifier proxies. This is often (though not always) combined with modeling work to better capture variation (as in \citealp{reidsma-carletta-2008-squibs}) or discussions of the limitations of this working hypothesis (as in \citeauthor{beigman-beigman-klebanov-2009-learning}).
% In other words, there are clear instances of the position we assume to be tenable being seriously considered — on empirical grounds, as a tentative explanation, or as a working hypothesis.
% We also stress that we politely disagree that this point is central to our claims — we highlight there are a a prima facie reasons for the position to be tenable in §2, and we effectively demonstrate that it empirically does not hold in §4, meaning those reasons are not valid. Compare with Baan et al who similarly criticize a position that is not made explicit by any one particular work.
}

==> miscellaneous.tex <==
% credit : https://scite.ai/assistant
The exploration of complexity and uncertainty in Natural Language Processing (NLP) is multifaceted, encompassing challenges arising from models, data, and human interactions. The literature identifies various underlying factors contributing to these complexities, which can be categorized into three primary domains: the intricacies of language itself, the limitations of computational models, and the variability in human language use.Firstly, the inherent complexity of human language presents significant challenges for NLP systems. Language is not merely a set of rules; it is a dynamic and context-dependent system influenced by cultural, social, and situational factors. This complexity is compounded by syntactic and semantic variations, which can lead to ambiguity and misinterpretation in NLP applications. For instance, the assessment of syntactic sophistication in second language writing illustrates how different methods can yield varying results, highlighting the nuanced nature of language that NLP must navigate (Kyle \& Crossley, 2017). Furthermore, the use of NLP in healthcare settings demonstrates the challenges posed by specialized vocabulary and complex semantics, where context is crucial for accurate interpretation (Parker, 2023; , Sadiku et al., 2018). These examples underscore the necessity for NLP systems to account for the multifaceted nature of language to reduce uncertainty in outcomes.Secondly, the limitations of computational models contribute to the uncertainty observed in NLP applications. While advancements in machine learning and deep learning have significantly improved NLP capabilities, these models often struggle with generalization across diverse datasets. For instance, the performance of models like BERT, which are pre-trained on specific corpora, may not translate effectively to other domains, such as clinical texts or informal communication (Crema et al., 2022). This limitation is exacerbated by the presence of noise in data, which can lead to misclassification and errors in understanding (Keogh et al., 2020). The literature emphasizes the importance of robust training datasets and the need for models to be adaptable to various contexts to mitigate these issues (Clarke et al., 2020). Consequently, the reliance on computational models introduces a layer of uncertainty that must be addressed through careful design and validation.Moreover, the interaction between NLP systems and human users introduces additional complexity. Human language is characterized by variability, including dialects, idiomatic expressions, and evolving usage patterns. This variability can lead to discrepancies between human understanding and machine interpretation, as evidenced by studies that highlight the differences in sentiment analysis outcomes when comparing human ratings to NLP-generated scores (Gratz et al., 2021). Furthermore, the integration of human feedback into NLP systems has been shown to enhance performance, suggesting that a collaborative approach can help bridge the gap between human language use and machine processing (Yu et al., 2021). However, this collaboration also introduces uncertainty, as human judgments can be subjective and influenced by personal biases.The literature also identifies several factors that contribute to the complexity and uncertainty in NLP, including data quality, model design, and the interpretability of results. Data quality is paramount; the presence of incomplete or biased data can skew results and lead to inaccurate conclusions (Iroju \& Olaleke, 2015). Additionally, the design of NLP models must consider the specific tasks they are intended to perform, as a one-size-fits-all approach may not yield optimal results across different applications (Shruthi \& Swamy, 2020). The interpretability of NLP systems is another critical factor, as stakeholders need to understand how decisions are made to trust and effectively use these technologies (Hollenstein et al., 2019). This need for transparency can further complicate the deployment of NLP systems in sensitive areas such as healthcare, where the stakes are high.In conclusion, the complexity and uncertainty inherent in NLP arise from a confluence of factors related to language intricacies, computational limitations, and human interactions. The literature underscores the importance of addressing these challenges through improved model design, robust data practices, and collaborative approaches that incorporate human insights. As NLP continues to evolve, ongoing research will be essential to refine these systems and enhance their reliability and effectiveness across diverse applications.

References:
Clarke, N., Foltz, P., & Garrard, P. (2020). How to do things with (thousands of) words: computational approaches to discourse analysis in alzheimer's disease. Cortex, 129, 446-463. https://doi.org/10.1016/j.cortex.2020.05.001
Crema, C., Attardi, G., Sartiano, D., & Redolfi, A. (2022). Natural language processing in clinical neuroscience and psychiatry: a review. Frontiers in Psychiatry, 13. https://doi.org/10.3389/fpsyt.2022.946387
Gratz, O., Vos, D., Burke, M., & Soares, N. (2021). Assessment of agreement between human ratings and lexicon-based sentiment ratings of open-ended responses on a behavioral rating scale. Assessment, 29(5), 1075-1085. https://doi.org/10.1177/1073191121996466
Hollenstein, N., Barrett, M., Troendle, M., Bigiolli, F., Langer, N., & Zhang, C. (2019). Advancing nlp with cognitive language processing signals.. https://doi.org/10.48550/arxiv.1904.02682
Iroju, O. and Olaleke, J. (2015). A systematic review of natural language processing in healthcare. International Journal of Information Technology and Computer Science, 7(8), 44-50. https://doi.org/10.5815/ijitcs.2015.08.07
Keogh, R., Shaw, P., Gustafson, P., Carroll, R., Deffner, V., Dodd, K., … & Freedman, L. (2020). Stratos guidance document on measurement error and misclassification of variables in observational epidemiology: part 1—basic theory and simple methods of adjustment. Statistics in Medicine, 39(16), 2197-2231. https://doi.org/10.1002/sim.8532
Kyle, K. and Crossley, S. (2017). Assessing syntactic sophistication in l2 writing: a usage-based approach. Language Testing, 34(4), 513-535. https://doi.org/10.1177/0265532217712554
Parker, R. (2023). Natural language processing enhanced qualitative methods: an opportunity to improve health outcomes. International Journal of Qualitative Methods, 22. https://doi.org/10.1177/16094069231214144
Sadiku, M., Zhou, Y., & Musa, S. (2018). Natural  language  processing  in  healthcare. International Journal of Advanced Research in Computer Science and Software Engineering, 8(5), 39. https://doi.org/10.23956/ijarcsse.v8i5.626
Shruthi, J. and Swamy, S. (2020). A prior case study of natural language processing on different domain. International Journal of Electrical and Computer Engineering (Ijece), 10(5), 4928. https://doi.org/10.11591/ijece.v10i5.pp4928-4936
Yu, S., Le, A., Feld, E., Schriver, E., Gabriel, P., Doucette, A., … & Mowery, D. (2021). A natural language processing–assisted extraction system for gleason scores: development and usability study. Jmir Cancer, 7(3), e27970. https://doi.org/10.2196/27970


%====================================================================

In the realm of Natural Language Processing (NLP), complexity and uncertainty are critical challenges that arise from various sources, including the models employed, the data utilized, and the inherent unpredictability of human language. The literature identifies several underlying causes contributing to these complexities and uncertainties.One significant source of uncertainty in NLP stems from the models themselves. Recent advancements in Bayesian deep learning have highlighted the importance of quantifying model uncertainties, which is essential for developing explainable and accountable AI systems. Xiao and Wang emphasize that understanding both model and data uncertainties can enhance the performance of NLP tasks, suggesting that reliable uncertainty quantification is a foundational step in building robust NLP applications (Xiao & Wang, 2019). Furthermore, the exploration of predictive uncertainty in NLP reveals that the quality of uncertainty estimates can be heavily influenced by the methodologies employed and the availability of data. For instance, Ulmer et al. found that while pre-trained models generally yield better uncertainty estimates, the quality can paradoxically decline with increased data availability, indicating a complex relationship between data volume and model performance (Ulmer et al., 2022). Data scarcity is another critical factor contributing to uncertainty in NLP. The field has predominantly focused on high-resource languages, leaving many languages underrepresented. This disparity leads to significant challenges in developing effective NLP models for low-resource languages, as highlighted by Aji et al., who argue that not only data scarcity but also the linguistic diversity and complexity of these languages contribute to the difficulties faced in NLP (Aji et al., 2022). The impact of data scarcity is further explored by Landeghem et al., who note that the heterogeneity of data can complicate the training of models, thereby increasing uncertainty in predictions (Landeghem et al., 2022). Human factors also play a crucial role in the complexity and uncertainty of NLP systems. The variability in human language—stemming from dialects, idioms, and cultural contexts—adds layers of complexity that models must navigate. This complexity is compounded by the fact that human language is often ambiguous and context-dependent, making it challenging for models to achieve high accuracy consistently. As noted by Yadav, the introduction of transformer models has significantly improved NLP performance, yet the inherent complexity of human language remains a formidable barrier (Yadav, 2024). Additionally, the unpredictability of human behavior and language use can lead to unforeseen challenges in NLP applications, particularly in tasks involving sentiment analysis or conversational agents.In summary, the complexity and uncertainty in NLP arise from a confluence of factors related to model architecture, data characteristics, and human language variability. Understanding these underlying causes is essential for advancing the field and improving the reliability of NLP systems. References: Aji, A., Winata, G., Koto, F., Cahyawijaya, S., Romadhony, A., Mahendra, R., … & Ruder, S. (2022). One country, 700+ languages: nlp challenges for underrepresented languages and dialects in indonesia.. https://doi.org/10.18653/v1/2022.acl-long.500 Landeghem, J., Blaschko, M., Anckaert, B., & Moens, M. (2022). Benchmarking scalable predictive uncertainty in text classification. Ieee Access, 10, 43703-43737. https://doi.org/10.1109/access.2022.3168734 Ulmer, D., Frellsen, J., & Hardmeier, C. (2022). Exploring predictive uncertainty and calibration in nlp: a study on the impact of method &amp; data scarcity.. https://doi.org/10.18653/v1/2022.findings-emnlp.198 Xiao, Y. and Wang, W. (2019). Quantifying uncertainties in natural language processing tasks. Proceedings of the Aaai Conference on Artificial Intelligence, 33(01), 7322-7329. https://doi.org/10.1609/aaai.v33i01.33017322 Yadav, A. (2024). Generative ai in the era of transformers: revolutionizing natural language processing with llms. Journal of Image Processing and Intelligent Remote Sensing, (42), 54-61. https://doi.org/10.55529/jipirs.42.54.61


